Beam Charge Asymmetries for Deeply Virtual Compton Scattering on the Proton at CLAS12

The parameterization of the nucleon structure through Generalized Parton Distributions (GPDs) shed a new light on the nucleon internal dynamics. For its direct interpretation, Deeply Virtual Compton Scattering (DVCS) is the golden channel for GPDs investigation. The DVCS process interferes with the Bethe-Heitler (BH) mechanism to constitute the leading order amplitude of the $eN \to eN\gamma$ process. The study of the $ep\gamma$ reaction with polarized positron and electron beams gives a complete set of unique observables to unravel the different contributions to the $ep \gamma$ cross section. This separates the different reaction amplitudes, providing a direct access to their real and imaginary parts which procures crucial constraints on the model dependences and associated systematic uncertainties on GPDs extraction. The real part of the BH-DVCS interference amplitude is particularly sensitive to the $D$-term which parameterizes the Gravitational Form Factors of the nucleon. The separation of the imaginary parts of the interference and DVCS amplitudes provides insights on possible higher-twist effects. We propose to measure the unpolarized and polarized Beam Charge Asymmetries (BCAs) of the $\vec{e}^{\pm}p \to e^{\pm}p \gamma$ process on an unpolarized hydrogen target with {\tt CLAS12}, using polarized positron and electron beams at 10.6 GeV. The azimuthal and $t$-dependences of the unpolarized and polarized BCAs will be measured over a large $(x_B,Q^2)$ phase space using a 100 day run with a luminosity of 0.66$\times 10^{35}$cm$^{-2}\cdot$s$^{-1}$.

==> App-Pos.tex <==
%
%------------------------------------------------------------------------------
%
% e+@CLAS12 Proposal to PAC51
%
% Polarized positron beams at Jefferson Lab
%
%------------------------------------------------------------------------------
%

\newpage

%
%------------------------------------------------------------------------------
%
\section{Polarized positron beams at Jefferson Lab}
\label{App-B}

The exploration of the full physics potential of the CEBAF 12 GeV would uniquely benefit from polarized and unpolarized positron beams with quality and modes of operation similar to those of the polarized electron beam.  The JLab Positron Working Group, formed in 2018 and now with over 250 members from 75 institutions, continues to build out a case to support this cause, and has explored an experimental program with high duty-cycle positron beams~\cite{Acc21}. Concurrently, the Ce$^+$BAF Working Group developed the concept of a new positron injector~\cite{Hab22} to support this physics program. A comprehensive R\&D program has been settled~\cite{ASy23,Gra23,Kaz23,Ush23} which current status is briefly reported in this appendix.

\subsection{Polarized positron beam production}

The creation of positron beams with a high degree of spin polarization is a challenging endeavour. At JLab, we can take advantage of the unique source of polarized electrons~\cite{Add10} and transfer their polarization to the positrons of $e^+e^-$-pairs created by the bremsstrahlung photons of the electrons inside a high-$Z$ target. This so-called PEPPo (Polarized Electrons for Polarized Positrons) technique was successfully demonstrated at the CEBAF injector using a 8.9~MeV/$c$ highly polarized electron beam, resulting in positron polarization up to 82\%~\cite{Abb16}. Most importantly, this technique is essentially independent of the initial electron beam energy, providing great flexibility to establish the positron yield which determines the positron beam intensity. The current design~\cite{Gra23} involves an initial electron beam of 120~MeV with an intensity of 1~mA and a polarization of 80\%.

\subsection{Positron injector concept}

\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.80\textwidth]{Figures/MOPL152_f2.pdf}
\end{center}
\caption{Layout of the polarized electron and positron injectors at LERF~\cite{Gra23}.}
\label{fig-PosInj}
\end{figure}
The present scheme takes advantage of the infrastructure of the Low Energy Research Facility (LERF) to install a new positron injector (Fig.~\ref{fig-PosInj}).

The existing LERF injector provides the baseline layout with the superconducting quarter cryomodule (Capture Linac: SRF 10 MV) capable of accelerating up to 10~mA Continuous Wave (CW) beams to 9~MeV/$c$~\cite{Her04}. A compact polarized electron source is installed upstream of the Capture Linac, including the electron gun followed by a Wien spin rotator and a buncher cavity for longitudinal matching to the SRF 10 MV. Downstream of the SRF 10 MV, a three dipole magnet chicane injects the electron beam into the first of two full-length accelerating SRF (Superconducting Radio Frequence) cryomodules (CM), 60~MV each. The electron gun will be a scaled-up version of the 130~keV inverted geometry gun used at CEBAF for many years~\cite{Add10}. It will be designed to operate at 300-350~kV and to accomodate larger laser beam spot size. This allows to manage higher bunch charges while extending the charge lifetime of the photo-cathode, and enables a direct injection to the SRF 10 MV. The final section of the electron injector shapes the transverse emittance to match the acceptance for two CEBAF style cryomodules which accelerate the beam energy to about 120~MeV. 

\begin{table}[!h]
\begin{center}
\begin{tabular}{lrrr}
\hline\hline
\textbf{Ce$^+$BAF Parameter} & \textbf{Status} &  \textbf{Goal}  \\ \hline
$p_0$ [MeV/$c$] & 60 & 60 \\
$\sigma_{\delta p/p_0}$ [\%] &    \color{black}{0.68} &  $\pm$1                \\
$\sigma_{z}$ [ps] &    \color{black}{3} &              $\leq 4$    \\     
Normalized $\epsilon_{n}$ [mm~mrad]  &  \color{black}{140}                & $\leq 40$ \\
 $p_f$ [MeV/$c$] & \color{black}{123} & 123 \\ $I_{\mathrm{e}^+} (P>60$\%) [nA] & \color{black}{170} & $>50$ \\  
\hline\hline
\end{tabular} 
\end{center}
\caption{Simulated parameters of the Ce$^+$BAF injector.}
\label{ce+bafparam}
\end{table}
The electron beam is further extracted to the positron radiator (High Power Target) which consists of a 4~mm thick water cooled tungsten target in form of a disk rotating at a moderate frequency of 2~Hz. This configuration allows to dissipate safely the 17~kW beam power deposited in the target~\cite{Ush23}. The generation of positrons in this thick target creates an exceptionally broad distribution in transverse and longitudinal phase space. A high field ($B_1$) quarter-wave transformer (QWT) located after the target decreases the transverse angular divergence of the positron distribution while also defining the central momentum of the positron polarization distribution to be collected. Following the high field region a low field ($B_2$) solenoid is used to manage the positron beam through an RF capture section which allows to decrease the longitudinal energy spread as well as to improve the transverse beam emittance. \newline
Following the RF capture region the positron momenta is defined by a chicane beamline composed of quadrupoles and dipoles to create a correlation between positron energy and transverse position at its midpoint where a collimator is installed. At the exit of the chicane a SRF CM accelerates positrons to 123~MeV, the required injection energy for CEBAF 12~GeV. A bunch compression chicane after the accelerating section achieves a bunch length of a few picoseconds. The final element of the positron injector is a high-energy spin rotator intented to orientate the spin of the positron beam in the direction appropriate for experiments after CEBAF acceleration. \newline
Results of recent CW polarized positron beam simulations are shown in Table~\ref{ce+bafparam} relative to our present design goals. All goals are exceeded except for the normalized emittance, which can be met by reducing the acceptance and compensating the resulting positron beam current reduction by increasing the drive beam power.

\subsection{Positron beam integration}

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.80\textwidth]{Figures/MOPL152_f1.pdf}
\end{center}
\caption{CEBAF and LERF accelerators. Green line shows the new 123~MeV transport beam line connecting LERF to CEBAF for high energy acceleration of positron beams~\cite{Gra23}.}
 \label{fig-PosInt}
\end{figure}
Once the CW positron beam has been formed and the spin oriented it is ready for acceleration to higher energies. Therefore, it should be transported form the LERF to the entrance of the North LinAc where electron beams are currently injected. \newline
A new tunnel connects the east side of LERF to the south east corner of CEBAF near the entrance of the South LinAc (Fig.~\ref{fig-PosInt}). This new beamline is designed to maintain small dispersion and to bring the beam to the elevation of the CEBAF South LinAc tunnel near the ceiling. Then a long FODO channel attached to the ceiling of the South Linac transports the beam to the west side of CEBAF where it is bent 180 degrees. At the end of this long transport line a vertical achromat translator and horizontal bending magnets bring the beam to the start of the North Linac where it is injected.

The CEBAF accelerator limits the maximum transverse emittance that can be transported. It is estimated that a normalized emittance between 40 and 120 mm.mrad can be accepted at the front of the North LinAc. In terms of longitudinal acceptance, the change of the optics configuration of the first two recirculation arcs for smaller dispersion functions will allow to inject up to a percent of energy spread in the front of the North LinAc and to transport a beam with a longitudinal bunch length around 1~mm.

\phantom{EmptyLine}

In brief, the Ce$^+$BAF working group has developed a scheme to provide CEBAF with polarized positron beams with CW time structure. Early designs and simulated parameters combined with constraints are approaching the anticipated goals. A broader document discussing in greater detail the technical approach and additional issues to be addressed is anticipated for the end of the current calendar year.
 
%
%------------------------------------------------------------------------------
%


==> Figures/e+C-Sys.tex <==
%
%------------------------------------------------------------------------------
%
% e+@CLAS12 Proposal to PAC48
%
% Control of systematic uncertainties
%
%------------------------------------------------------------------------------
%

\section{Control of systematic uncertainties}
\label{sec:sys}

\subsection{Origin of systematic effects}

Systematic effects can occur on the one hand from positron beam properties, and on the other hand from the response of the {\tt CLAS12} spectrometer. 

\begin{figure}[!h]
\begin{center}
\includegraphics[width=0.50\columnwidth]{Figures/CLAS12-side.png}
\caption{The generic setup of the {\tt CLAS12} detector in Hall B in a side view. For the same kinematics the forward going particles electrons and positrons are following the same path for reversed polarity of the Torus magnet and the solenoid magnet (both bending away from the beam line).} 
\label{CLAS12-side}
\end{center}
\end{figure} 
The expected positron beam properties in the physics interaction region differ from the CEBAF electron beam essentially by a 4-5 times larger emittance. Additional focusing of the beam will be provided by a set of quadrupoles already installed on the beam line but residual effects of the beam properties difference may remain which could alter the comparison with electron data. To control these effects DVCS data with an electron beam having the same properties as the positron beam should be carried out. Such beam can be made out of the secondary electrons produced at the positron source, which is expected to have similar properties in terms of $(x,y)$ profile and emittance at the  target position. This will allow for the elimination/correction of potential beam-related false asymmetries.

Systematic uncertainties for DVCS cross section measurements with electron beams are part of the currently ongoing program with the {\tt CLAS12} spectrometer setup. For positron beams most of these systematic effects are very similar as far as the {\tt CLAS12} detector properties and normalization issues are concerned. As we aim for measurements of charge differences in cross sections or charge asymmetries most of them will be identical and will therefore drop out in the difference of electron and positron measurements. There are a few effects that however may not drop out and have to be considered.

The experimental setup is generically shown in a side view in Fig.~\ref{CLAS12-side}, and in  Fig.~\ref{clas12-cartoon} in a view along the beam line looking downstream. For the scattered positron and for the DVCS photon the detector looks identical to the situation when electrons are scattered off protons and the magnetic fields in both magnets are reversed. Additional software fiducial cuts will further ensure the same detector status between electron and positron data taking for these particles driving the resolution of the DVCS analysis. This is not the case of the recoil proton, which will be bent in the solenoid field in the opposite direction compared to the electron scattering case. This could result in systematic effects due to potentially different track reconstruction efficiencies and effective solid angles. While these effects are much smaller than the physics asymmetry (see Sec.~\ref{Sec:BCA}), we propose here to measure the positron DVCS process 50\% of the time with reversed solenoid polarity so that the proton will bend half time in one direction and half time in the opposite direction. \newline
Another cross check is possible by measuring the elastic $e^+p \to e^+p$ scattering cross section continuously during the experiments. The {\tt CLAS12} acceptance covers elastic scattering and deep inelastic processes, such as DVCS, and both will be measured concurrently. In either case most of the recoil protons are detected in the central detector, giving us continuous control of the performance of the detector system throughout the experiment. It should be noted that the elastic $e^+p \to e^+p$ cross section is equal to the well known elastic $e^-p \to e^-p$ cross section within the contributions from 2-photon effects, which are very small in the kinematic range that can be selected for the process~\cite{Afa17}.  
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.75\columnwidth]{Figures/clas12-central.jpg}
\caption{The generic setup of the {\tt CLAS12} detector in Hall B viewed from upstream down the beam pipe. In this view the proton rotates in the opposite direction, from the case of the electron beam. When swithing the solenoid field the electron and positron experience different phi motions due to the opposite motion of electron and positrons (left). When the solenoid field is reversed the electrons and positrons get kicks in the opposite azimuthal directions as seen that positrons and electrons switch place in the forward detector. This potential asymmetry can be controlled with elastic scattered electrons and positrons.} 
\label{clas12-cartoon}
\end{center}
\end{figure} 

The charge asymmetries for the DVCS process can be large (see Sec.~\ref{Sec:BCA}). From the simulation calibrated by the measurement of known processes, we aim at keeping systematic uncertainties due to these effects below 3\% at all kinematics. We also note that for the positron beam spin asymmetry, which will be measured concurrently, the systematic uncertainties are not affected by the aforementioned electron-positron differences. 

\subsection{Beam charge asymmetry systematics}

The unpolarized raw Yield Charge Asymmetry (YCA) is defined experimentally as
\begin{equation}
\mathcal{Y}^C_{UU} = \frac{(Y^+_+ + Y^+_-) - (Y^-_+ + Y^-_-)}{Y^+_+ + Y^+_- + Y^-_+ + Y^-_-}
\end{equation}
where 
\begin{equation}
Y^e_{\lambda} = \frac{N^e_{\lambda}}{Q^e_{\lambda}} = n^e_{\lambda}
\end{equation}
is the beam charge and spin dependent normalized yield determined from the number of events $N^e_{\lambda}$ and the corresponding accumulated charge $Q^e_{\lambda}$. Comparing electron and positron measurements taken at different periods of time, the detector may not be exactly the same. This translates into different efficiencies ($\epsilon^e$) and solid angles ($\Delta \Omega^e$) leading to an excess/deficit of positron events as compared to the true physics event number expected within the acceptance of electron beam data. Noting $\delta n^0_0$ the spin and charge independent positron excess, the charge normalized yield for electrons and positrons can be expressed as
\begin{eqnarray}
n^-_{\pm} & = & n^0_0 \left[ 1 - A^C_{UU} \pm \left( A^0_{LU} - A^C_{LU}\right) \right] \\
n^+_{\pm} & = & n^0_0 \left( 1 + \frac{\delta n^0_0}{n^0_0} \right) \, \left[ 1 + A^C_{UU} \pm \left( A^0_{LU} + A^C_{LU}\right) \right] 
\end{eqnarray}
where $n_0^0$ is the unpolarized normalized neutral yield for identical detectors and the $A^i_{jk}$ are the physics BCAs. The detector difference is represented by the ratio
\begin{equation}
\frac{\epsilon^+ \Delta \Omega^+}{\epsilon^- \Delta \Omega^-} = 1 + \frac{\delta n_0^0}{n^0_0} = 1 + 2 \eta_C = 1 + 2 \left( C_{\epsilon} + C_{\Delta\Omega} + 2 C_{\epsilon} C_{\Delta\Omega} \right)
\end{equation}
where $\eta_C$ is the detector correction which involves the efficiency and solid angle relative differences
\begin{eqnarray}
C_{\epsilon} & = & \frac{1}{2} \, \frac{\Delta_{\epsilon}}{\epsilon^-} = \frac{1}{2} \, \frac{\epsilon^+ - \epsilon^-}{\epsilon^-} \\ 
C_{\Delta\Omega}  & = & \frac{1}{2} \, \frac{\Delta_{\Delta\Omega}}{\Delta \Omega^-} = \frac{1}{2} \, \frac{\Delta \Omega^+ - \Delta \Omega^-}{\Delta \Omega^-} \, .
\end{eqnarray}
The unpolarized physics BCA, taking into account detector difference effects, can be derived from the experimental YCA following the expression 
\begin{equation}
A^C_{UU} = \frac{\left( 1 + \eta_C \right) \, \mathcal{Y}^C_{UU} - \eta_C}{1 + \eta_C - \eta_C \, \mathcal{Y}^C_{UU}} \, . \label{ACuu:YCUU}
\end{equation}
Similarly, the polarized raw YCAs are defined as
\begin{eqnarray}
\mathcal{Y}^C_{LU} & = & \frac{(Y^+_+ - Y^+_-)/\lambda^+ - (Y^-_+ - Y^-_-)/\lambda^-}{Y^+_+ + Y^+_- + Y^-_+ + Y^-_-} \\
\mathcal{Y}^0_{LU} & = & \frac{(Y^+_+ - Y^+_-)/\lambda^+ - (Y^-_+ - Y^-_-)/\lambda^-}{Y^+_+ + Y^+_- + Y^-_+ + Y^-_-}
\end{eqnarray}
from which the polarized physics BCAs, considering detector difference effects, are obtained as  
\begin{eqnarray}
A^C_{LU} & = & \frac{(1+\eta_C) \mathcal{Y}^C_{LU} - \eta_C \mathcal{Y}^0_{LU}}{1+\eta_C-\eta_C \, \mathcal{Y}^C_{UU}} \approx \frac{(1+2\eta_C) \mathcal{Y}^C_{LU}}{1+\eta_C-\eta_C \, \mathcal{Y}^C_{UU}} \label{ACLu:YCLU} \\
A^0_{LU} & = & \frac{(1+\eta_C) \mathcal{Y}^0_{LU} - \eta_C \mathcal{Y}^C_{LU}}{1+\eta_C-\eta_C \, \mathcal{Y}^C_{UU}} \approx 0 \label{A0Lu:Y0LU}
\end{eqnarray}
where the approximation holds at twist-2. Because of possible detector asymmetry effects bewteen beams of opposite charge, polarized BCAs combine unpolarized and polarized raw asymmetries. Thanks to the polarity reversal of the {\tt CLAS12} magnets, the magnitude of these effects will be minimized and it is reasonable to expect differences smaller than 10\%, corresponding to the hypotheses $C_{\epsilon}$$\le$0.05 and $C_{\Omega}$$\le$0.05. The precision on these corrections directly enters the systematic error on BCAs, which is determined as
\begin{equation}
\delta \left[ A^C_{UU} \right]_{Sys.} = \sqrt{ {\left( \frac{dA^C_{UU}}{dC_{\epsilon}} \, \delta \left[ C_{\epsilon} \right] \right)}^2 + {\left( \frac{dA^C_{UU}}{dC_{\Delta\Omega}} \, \delta \left[ C_{\Delta\Omega} \right] \right)}^2 } \, 
\end{equation}
and similarly for polarized BCAs. Considering that the systematic of the efficiency ($\Delta_{\epsilon}$) and solid angle ($\Delta_{\Delta\Omega}$) differences is independent of the absolute knowledge of the efficiency and of the solid angle, we have 
\begin{eqnarray}
\delta C_{\epsilon} & = & \vert C_{\epsilon} \vert \, \sqrt{\left( \frac{\delta \Delta_{\epsilon}}{\Delta_{\epsilon}} \right)^2 + \left( \frac{\delta \epsilon^-}{\epsilon^-} \right)^2 } \\
\delta C_{\Delta\Omega} & = & \vert C_{\Delta\Omega} \vert \, \sqrt{\left( \frac{\delta \Delta_{\Delta\Omega}}{\Delta_{\Delta\Omega}} \right)^2 + \left( \frac{\delta \Delta\Omega^-}{\Delta\Omega^-} \right)^2 } \, .
\end{eqnarray}
The magnitude of the corrections to raw unpolarized and polarized YCAs are determined as the deviation from the physics BCAs. The left panel of Fig.~\ref{Sys_BCA} reports the envelope of the possible corrections assuming $C_{\epsilon}$ and $C_{\Delta\Omega}$ values within $\pm$0.05 (or $\pm$0.02). The right panel of Fig.~\ref{Sys_BCA} reports  within the same conditions the envelope of systematic errors related to efficiency and solid angle corrections assuming 3\% systematic uncertainty on $\Delta_{\epsilon}$ and 7\% systematic uncertainty on $\epsilon^{-}$, and similarly for the solid angle correction. Under these assumptions, the absolute systematic uncertainties on unpolarized BCA are smaller than 0.01. 


\newpage

\null\vfill

\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.9\textwidth]{Figures/Sys_BCA.pdf}
\includegraphics[width=0.9\textwidth]{Figures/Sys_BCLA.pdf}
\includegraphics[width=0.9\textwidth]{Figures/Sys_B0LA.pdf}
%\caption{Amplitude of the corrections of unpolarized raw asymmetries (left) and of the corresponding systematic error on unpolarized BCA (right). The shaded areas indicate the possible values of the corrections for a fixed raw asymmetry assuming that the efficiency and solid angle corrections are comprised within $\pm$5\% (solid line) and $\pm$2\% (dashed line). Asymmetry systematics is evaluated assuming 3.5\% relative uncertainty on efficiency and solid angles. Amplitude of the corrections of polarized raw asymmetries (left) and of the corresponding systematic error on polarized BCA (right). The shaded areas indicate the possible values of the corrections for a fixed raw asymmetry assuming that the positron BSA is comprised within $\pm$50\%, and that the efficiency and solid angle corrections take values within $\pm$5\% (solid line) and $\pm$2\% (dashed line). The solid black line limits the variation domain when the positron BSA is comprised within $\pm$25\%. Asymmetry systematics is evaluated assuming a 3.5\% relative uncertainty on efficiency and solid angles.}
\label{Sys_BCA}
\end{center}
\end{figure}

\vfill\eject

The magnitude of efficiency and solid angle corrections effects and related absolute systematic uncertainties for polarized BCA is determined using the same approach as in the upolarized case. According to Eq.~\ref{ACLu:YCLU}, these are depending in addition on the positron BSA which is assumed to vary within $\pm$50\% (red curves) or $\pm$25\% (black curves). The absolute systematic uncertainty related to differences between electron and positron measurements may amount up to 0.06 in the case of large asymmetries.

The determination of the magnitude of the corrections of raw asymmetries and their attached systematics reported on Fig.~\ref{Sys_BCLA} is also valid for the neutral BSA. In the twist-2 approximation where the neutral BSA is predicted to be zero, systematics effects may account for up to 0.03 depending essentially on the magnitude of the positron BSA.

The effect of eventual efficiency and solid angle dissymmetries between electron and positron data taking can generally be sizeable but can be corrected for with high accuracy by calibrating simulations with specific measurements of a knwon physics process.

%
%------------------------------------------------------------------------------
%

